EROICA: Online Performance Troubleshooting for Large-scale Model Training

Troubleshooting performance problems of large model training (LMT) is immensely challenging, due to unprecedented scales of modern GPU clusters, the complexity of software-hardware interactions, and the data intensity of the training process. Existing troubleshooting approaches designed for traditional distributed systems or datacenter networks fall short and can hardly apply to real-world training systems. In this paper, we present EROICA, the first online troubleshooting system that provides both fine-grained observation based on profiling, and coverage of all machines in GPU clusters, to diagnose performance issues in production, including both hardware and software problems (or the mixture of both). EROICA effectively summarizes runtime behavior patterns of LMT function executions via online profiling, and leverages differential observability to localize the root cause with minimal production impact. EROICA has been deployed as a production service for large-scale GPU clusters of ~100,000 GPUs for 1.5 years. It has diagnosed a variety of difficult performance issues with 97.5% success.

==> sections/abs.tex <==
\begin{abstract}
Large model training (\dlt) brings about the critical challenge of performance diagnosis. To provide information for diagnosis, existing systems either operate online monitoring or offline profiling for hardware \& application-level operations. The former is light-weighted enough to be deployed online, but ignores fine-grained details which may be necessary for problem identification, while the latter provides detailed information but introduces huge overload, so it requires offline problem regeneration and experiments.

To combine the advantages of both, we present \sys, the first \dlt performance diagnosis system based on online profiling. \sys extracts function behavior patterns from the online profiling data, which can well-describe each worker's behavior during the function execution with limited data size. Then the performance diagnosis algorithm makes comparisons between these patterns, and outputs the abnormal function executions with their behaviors.
\sys has been deployed as a product in production GPU clusters of $O(10,000)$ GPUs, and helps our customers to identify various performance issues, improving \dlt performance.
\end{abstract}
